Predicting knee osteoarthritis severity: comparative modeling based on patient's data and plain X-ray images

Knee osteoarthritis (KOA) is a disease that impairs knee function and causes pain. A radiologist reviews knee X-ray images and grades the severity level of the impairments according to the Kellgren and Lawrence grading scheme; a five-point ordinal scale (0--4). In this study, we used Elastic Net (EN) and Random Forests (RF) to build predictive models using patient assessment data (i.e. signs and symptoms of both knees and medication use) and a convolution neural network (CNN) trained using X-ray images only. Linear mixed effect models (LMM) were used to model the within subject correlation between the two knees. The root mean squared error for the CNN, EN, and RF models was 0.77, 0.97, and 0.94 respectively. The LMM shows similar overall prediction accuracy as the EN regression but correctly accounted for the hierarchical structure of the data resulting in more reliable inference. Useful explanatory variables were identified that could be used for patient monitoring before X-ray imaging. Our analyses suggest that the models trained for predicting the KOA severity levels achieve comparable results when modeling X-ray images and patient data. The subjectivity in the KL grade is still a primary concern.

==> Research day/JNresearchday.tex <==


\author{\textbf{Newell, John}} % Name
\maketitle %don't delete
\abstract %don't delete

\subsubsection*{Current Research Interests} % 1 paragraph

My primary areas of research in Biostatistics are in the theory and application of statistical methods in clinical trials of 
health service and population health interventions and in the development of novel analytic approaches in Sports and Exercise Science.  
My research interests include statistical modelling, statistical computing, design and analysis of cluster randomised trials, 
smoothing techniques and derivative estimation, survival analysis, tree based classification problems and sports analytics.

\subsubsection*{Publications}
% Number of publications appearing in calender year 2018
6 publications appeared in calendar year 2018

Most significant recent publications %(up to 4)
\begin{enumerate}
\item    Ferguson, J,Alvarez-Iglesias, A,Newell, J,Hinde, J,O'Donnell, M. (2018), Estimating average attributable fractions with confidence intervals for cohort and case-control studies. Statistical Methods In Medical Research, 27 :1141-1152.
\item    Hayes P, Casey M, Glynn LG, Molloy GJ, Durand H, O'Brien E, Dolan E, Newell J, Murphy AW. (2018) Prevalence of treatment-resistant hypertension after considering pseudo-resistance and morbidity: a cross-sectional study in Irish primary care'. British Journal Of General Practice, 68 (671):394-400.
\item    Molloy GJ, Noone C, Caldwell D, Welton NJ, Newell J (2018) Network meta-analysis in health psychology and behavioural medicine: a primer. Health Psychology Review.
\item    Hayes P, Kielty H, Casey M, Glynn LG, Molloy GJ, Durand H, Newell J, Murphy AW (2018) 'Prognosis of patients with apparent treatment-resistant hypertension-a feasibility study'. Pilot and Feasibility Studies, 43.
\end{enumerate}


\subsubsection*{Research Activities} % 1 paragraph covering calender year 2018.

\begin{itemize}
\item Current research grants: PI (1), Co-PI (2), Co-Applicant (3).
\item Graduate students: Davood Roshan, Kishor Das, Jaynal Abedin (Insight), Lara Coyne (Insight), Diarmuid Daniels (Insight).
\item Journal submissions: 9
\item Conferences: Organised 31st Conference on Applied Statistics in Ireland (CASI), Galway May 2018.
\item Research Visits: St Mary's University Twickenham.
\item Invited talks: 1
\item Memberships: International Society for Clinical Biostatistics, Irish Statistical Association
\item External posts: Adjunct Senior Research Fellow in the Department of Mathematics and Statistics, University of Canterbury, Christchurch, New Zealand.
\end{itemize}

% This might include: Current research grants, numbers of graduate students, journal submissions, conferences, visits, invited talks, research visits, papers refereed, math reviews, editorships, memberships, external posts, etc






